P.A.M. Dirac and the Discovery of Quantum Mechanics

This colloquium summarizes Dirac's contributions to the discovery of quantum mechanics before he invented his relativistic wave equation.

==> FontMacros-12.tex <==
% FILENAME: FontMacros-12/99-KG
% (12/9/99)
\usepackage[psamsfonts]{amssymb}

\makeatletter

% This package just makes labels appear near the equation numbers

\RequirePackage{amsmath}[1995/02/23]
\DeclareOption{logtags}{\l@gtagstrue}

\newif\ifl@gtags \l@gtagsfalse
\ProcessOptions

\let\saved@tagform@\tagform@
\def\tagform@#1{%
   \ifl@gtags\typeout{[equation\space(#1)=\df@label]}\fi%
   \iftagsleft@%
      \saved@tagform@{\llap{{\small\df@label}\kern6pt}#1}%
   \else%
      \saved@tagform@{#1\rlap{\kern6pt{\small\df@label}}}%
   \fi}

\makeatother

% BASIC MACROS

\newcommand{\al}{\alpha}
\newcommand{\bet}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\Gam}{\Gamma}
\newcommand{\eps}{\epsilon}
\newcommand{\del}{\delta}
\newcommand{\lam}{\lambda}
\newcommand{\Lam}{\Lambda}
\newcommand{\kap}{\kappa}
\newcommand{\sig}{\sigma}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\Sig}{\Sigma}
\newcommand{\Del}{\Delta}
\newcommand{\Ups}{\Upsilon}


\newcommand{\mr}{\mathrm}
\newcommand{{\smfrac}}{{\scriptstyle\frac}}
\newcommand{\h}{\hbar}
\newcommand{\lb}{[}
\newcommand{\rb}{]}
\newcommand{\diff}{\partial}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bra}{\langle}
\newcommand{\ket}{\rangle}
\newcommand{\lsim}{\lesssim}
\newcommand{\gsim}{\gtrsim}
\newcommand{\half}{{\scriptstyle\frac{1}{2}}}
\newcommand{\shalf}{{\scriptscriptstyle\frac{1}{2}}}
\newcommand{\third}{{\scriptstyle\frac{1}{3}}}
 \newcommand{\sthird}{{\scriptscriptstyle\frac{1}{3}}}
\newcommand{\quarter}{{\scriptstyle\frac{1}{4}}}
\newcommand{\sthalf}{{\scriptscriptstyle\frac{3}{2}}}
%\newcommand{\s13}{{\script\scriptstyle\frac{1}{3}}}
%\newcommand{\s14}{{\script\scriptstyle\frac{1}{4}}}
%\newcommand{\s23}{{\script\scriptstyle\frac{1}{3}}}
\newcommand{\sdag}{{\scriptstyle \dagger}}
\newcommand{\tm}{\times}
\newcommand{\non}{\nonumber}
\newcommand{\rar}{\rightarrow}
\newcommand{\Lrar}{\longrightarrow}
\newcommand{\lrar}{\leftrightarrow}
\newcommand{\uar}{\uparrow}
\newcommand{\dar}{\downarrow}
\newcommand{\vphi}{\varphi}
\newcommand{\vrho}{\varrho}
\newcommand{\vreps}{\varepsilon}
\newcommand{\vtheta}{\vartheta}

\newcommand{\Tr}{{\rm Tr}\,}
\newcommand{\Det}{{\rm det}}
%\renewcommand{\par}{\!\parallel\!}

% INTEGRALS

\newcommand{\I}{\int_{-\infty}^{\infty}}
\newcommand{\J}{\int_{0}^{\infty}}



\newcommand{\bs}[1]{{\boldsymbol{#1}}}

\renewcommand{\cal}[1]{{\mathcal{#1}}}

%BOLDFACE: nabla, dot and cross products

%\newcommand{\B}{{\bs{}}}

\newcommand{\Bnabla}{{\boldsymbol{\nabla}}}

\newcommand{\Bdotn}{{\bs{\cdot}}}
\newcommand{\Bdot}{{\,\bs{\cdot}\,}}
\newcommand{\Btm}{{\bs{\tm}}}

%CALIGRAPHIC

%\newcommand{}{}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}


%BOLDFACE ITALICS:

\newcommand{\BA}{{\bs{A}}}
\newcommand{\Ba}{{\bs{a}}}
\newcommand{\BB}{{\bs{B}}}
\newcommand{\Bb}{{\bs{b}}}
\newcommand{\BC}{{\bs{C}}}
\newcommand{\Bc}{{\bs{c}}}
\newcommand{\BD}{{\bs{D}}}
\newcommand{\Bd}{{\bs{d}}}
\newcommand{\BE}{{\bs{E}}}
\newcommand{\Be}{{\bs{e}}}
\newcommand{\BF}{{\bs{F}}}
\newcommand{\Bf}{{\bs{f}}}
\newcommand{\BG}{{\bs{G}}}
\newcommand{\Bg}{{\bs{g}}}
\newcommand{\BH}{{\bs{H}}}
\newcommand{\Bh}{{\bs{h}}}
\newcommand{\BI}{{\bs{I}}}
\newcommand{\Bi}{{\bs{i}}}
\newcommand{\BJ}{{\bs{J}}}
\newcommand{\Bj}{{\bs{j}}}
\newcommand{\BK}{{\bs{K}}}
\newcommand{\Bk}{{\bs{k}}}
\newcommand{\BL}{{\bs{L}}}
\newcommand{\Bl}{{\bs{l}}}
\newcommand{\BM}{{\bs{M}}}
\newcommand{\Bm}{{\bs{m}}}
\newcommand{\BN}{{\bs{N}}}
\newcommand{\Bn}{{\bs{n}}}
\newcommand{\BO}{{\bs{O}}}
\newcommand{\BP}{{\bs{P}}}
\newcommand{\Bp}{{\bs{p}}}
\newcommand{\BQ}{{\bs{Q}}}
\newcommand{\Bq}{{\bs{q}}}
\newcommand{\BR}{{\bs{R}}}
\newcommand{\Br}{{\bs{r}}}
\newcommand{\BS}{{\bs{S}}}
\newcommand{\Bs}{{\bs{s}}}
\newcommand{\BT}{{\bs{T}}}
\newcommand{\Bt}{{\bs{t}}}
\newcommand{\BU}{{\bs{U}}}
\newcommand{\Bu}{{\bs{u}}}
\newcommand{\BV}{{\bs{V}}}
\newcommand{\Bv}{{\bs{v}}}
\newcommand{\BW}{{\bs{W}}}
\newcommand{\Bw}{{\bs{w}}}
\newcommand{\BX}{{\bs{X}}}
\newcommand{\Bx}{{\bs{x}}}
\newcommand{\BY}{{\bs{Y}}}
\newcommand{\By}{{\bs{y}}}
\newcommand{\BZ}{{\bs{Z}}}
\newcommand{\Bz}{{\bs{z}}}


% GREEK BOLDFACE

\newcommand{\Bal}{{\bs{\al}}}
\newcommand{\Bbet}{{\bs{\bet}}}
\newcommand{\Bgam}{{\bs{\gam}}}
\newcommand{\BGam}{{\bs{\Gam}}}
\newcommand{\Bdel}{{\bs{\del}}}
\newcommand{\BDel}{{\bs{\Del}}}
\newcommand{\Beps}{{\bs{\eps}}}
\newcommand{\Bphi}{{\bs{\phi}}}
\newcommand{\BPhi}{{\bs{\Phi}}}
\newcommand{\Bxi}{{\bs{\xi}}}
\newcommand{\BXi}{{\bs{\Xi}}}
\newcommand{\Beta}{{\bs{\eta}}}
\newcommand{\Bzeta}{{\bs{\zeta}}}
\newcommand{\Btheta}{{\bs{\theta}}}
\newcommand{\BTheta}{{\bs{\Theta}}}
\newcommand{\Bkap}{{\bs{\kap}}}
\newcommand{\Blam}{{\bs{\lam}}}
\newcommand{\BLam}{{\bs{\Lam}}}
\newcommand{\Bmu}{{\bs{\mu}}}
\newcommand{\Bnu}{{\bs{\nu}}}
\newcommand{\Bpi}{{\bs{\pi}}}
\newcommand{\BPi}{{\bs{\Pi}}}
\newcommand{\Brho}{{\bs{\rho}}}
\newcommand{\Bsig}{{\bs{\sig}}}
\newcommand{\BSig}{{\bs{\Sig}}}
\newcommand{\Btau}{{\bs{\tau}}}
\newcommand{\Bvtheta}{{\bs{\vtheta}}}
\newcommand{\Bpsi}{{\bs{\psi}}}
\newcommand{\BPsi}{{\bs{\Psi}}}
\newcommand{\Bchi}{{\bs{\chi}}}
\newcommand{\Bom}{{\bs{\om}}}
\newcommand{\BOm}{{\bs{\Omega}}}






%\newcommand{\bfal}{\mbox{\boldmath $\alpha$}}
%\newcommand{\bfgam}{\mbox{\boldmath $\gam$}}
%\newcommand{\bfbet}{\mbox{\boldmath $\beta$}}
%\newcommand{\bfdel}{\mbox{\boldmath $\del$}}
%\newcommand{\bfeps}{\mbox{\boldmath $\eps$}}
%\newcommand{\bfzeta}{\mbox{\boldmath $\zeta$}}
%\newcommand{\bfeta}{\mbox{\boldmath $\eta$}}
%\newcommand{\bfkap}{\mbox{\boldmath $\kappa$}}
%\newcommand{\bfom}{\mbox{\boldmath $\om$}}
%\newcommand{\bflam}{\mbox{\boldmath $\lambda$}}
%\newcommand{\bfmu}{\mbox{\boldmath $\mu$}}
%\newcommand{\bfxi}{\mbox{\boldmath $\xi$}}
%\newcommand{\bfsig}{\mbox{\boldmath $\sigma$}}
%\newcommand{\bfpi}{\mbox{\boldmath $\pi$}}
%\newcommand{\bfrho}{\mbox{\boldmath $\rho$}}
%\newcommand{\bftau}{\mbox{\boldmath $\tau$}}





% BLACKBOARD CAPS

\newcommand{\bA}{{\mathbb{A}}}
\newcommand{\bC}{{\mathbb{C}}}
\newcommand{\bE}{{\mathbb{E}}}
\newcommand{\bB}{{\mathbb{B}}}
\newcommand{\bH}{{\mathbb{H}}}
\newcommand{\bK}{{\mathbb{K}}}
\newcommand{\bQ}{{\mathbb{Q}}}
\newcommand{\bR}{{\mathbb{R}}}
\newcommand{\bD}{{\mathbb{D}}}
\newcommand{\bF}{{\mathbb{F}}}
\newcommand{\bG}{{\mathbb{G}}}
\newcommand{\bI}{{\mathbb{I}}}
\newcommand{\bJ}{{\mathbb{J}}}
\newcommand{\bL}{{\mathbb{L}}}
\newcommand{\bM}{{\mathbb{M}}}
\newcommand{\bN}{{\mathbb{N}}}
\newcommand{\bP}{{\mathbb{P}}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bU}{{\mathbb{U}}}
\newcommand{\bV}{{\mathbb{V}}}
\newcommand{\bW}{{\mathbb{W}}}
\newcommand{\bX}{{\mathbb{X}}}
\newcommand{\bY}{{\mathbb{Y}}}
\newcommand{\bZ}{{\mathbb{Z}}}
\newcommand{\bO}{{\mathbb{O}}}


% EULER GOTHIC CAPS

\newcommand{\EC}{\mathfrak {C}}
\newcommand{\ED}{\mathfrak {D}}
\newcommand{\EE}{\mathfrak{E}}
\newcommand{\EH}{\mathfrak {H}}
\newcommand{\EG}{\mathfrak{G}}
\newcommand{\EP}{\mathfrak{P}}
\newcommand{\EQ}{\mathfrak{Q}}
\newcommand{\EA}{\mathfrak{A}}
\newcommand{\EB}{\mathfrak{B}}
\newcommand{\EF}{\mathfrak{F}}
\newcommand{\EK}{\mathfrak{K}}
\newcommand{\EL}{\mathfrak{L}}
\newcommand{\EM}{\mathfrak{M}}
\newcommand{\EN}{\mathfrak{N}}
\newcommand{\EO}{\mathfrak{O}}
\newcommand{\ER}{\mathfrak{R}}
\newcommand{\ES}{\mathfrak{S}}
\newcommand{\ET}{\mathfrak{T}}
\newcommand{\EU}{\mathfrak{U}}
\newcommand{\EV}{\mathfrak{V}}
\newcommand{\EW}{\mathfrak{W}}
\newcommand{\EX}{\mathfrak{X}}
\newcommand{\EY}{\mathfrak{Y}}
\newcommand{\EZ}{\mathfrak{Z}}
\newcommand{\EI}{\mathfrak{I}}
\newcommand{\EJ}{\mathfrak{J}}







 

